Dragoon: Private Decentralized HITs Made Practical

With the rapid popularity of blockchain, decentralized human intelligence tasks (HITs) are proposed to crowdsource human knowledge without relying on vulnerable third-party platforms. However, the inherent limits of blockchain cause decentralized HITs to face a few "new" challenges. For example, the confidentiality of solicited data turns out to be the sine qua non, though it was an arguably dispensable property in the centralized setting. To ensure the "new" requirement of data privacy, existing decentralized HITs use generic zero-knowledge proof frameworks (e.g. SNARK), but scarcely perform well in practice, due to the inherently expensive cost of generality. We present a practical decentralized protocol for HITs, which also achieves the fairness between requesters and workers. At the core of our contributions, we avoid the powerful yet highly-costly generic zk-proof tools and propose a special-purpose scheme to prove the quality of encrypted data. By various non-trivial statement reformations, proving the quality of encrypted data is reduced to efficient verifiable decryption, thus making decentralized HITs practical. Along the way, we rigorously define the ideal functionality of decentralized HITs and then prove the security due to the ideal-real paradigm. We further instantiate our protocol to implement a system called Dragoon, an instance of which is deployed atop Ethereum to facilitate an image annotation task used by ImageNet. Our evaluations demonstrate its practicality: the on-chain handling cost of Dragoon is even less than the handling fee of Amazon's Mechanical Turk for the same ImageNet HIT.

==> primitive.tex <==
   %!TEX root = main.tex

    \begin{figure}[!h]
	\centering
	\includegraphics[width=8.5cm]{primitive.eps}
	\caption{Subtle linkability of the \sameprefix-linkable anonymous authentication scheme. All involved algorithms except $\cSetup$ are shown in bold.}
	\label{fig:primitive}
	\end{figure}
   
   
    \subsection{Common-prefix-linkable anonymous authentication}  
    
    

    
    \label{sec:primitive}     
     Before the formal description of \system's protocol, let us introduce the new primitive for achieving the anonymous-yet-accountable authentication first. As briefly shown in Fig.\ref{fig:primitive}, our new primitive can be built atop any certification procedure, thus we include a certification generation procedure that can be inherited from any existing one. Also, we insist on {\em non-interactive} authentication, thus all the steps (including the authentication step) are described as algorithms instead of protocols. Formally, a common-prefix-linkable anonymous authentication scheme is composed of the following algorithms:
   
      \begin{enumerate}
      \item[-] $\cSetup(1^\lambda)$. This algorithm outputs the system's master public key $mpk$, and system's master secret key $msk$, where $\lambda$ is the security parameter.
      \item[-] $\cCertGen(msk,pk)$. This algorithm outputs a certificate $cert$ to validate the public key.
      \item[-] $\Auth(m,sk,pk,cert,mpk)$. This algorithm generates an attestation $\pi$ on a message $m$ that: the sender of $m$ indeed owns a secret key corresponding to a valid certificate.
      \item[-] $\Verify(m,mpk,\pi)$. This algorithm outputs $0/1$ to decide whether the attestation is valid or not.
      \item[-] $\Link(mpk,m_1,\pi_1,m_2,\pi_2)$. This algorithm takes  two valid message-attestation pairs, i.e. $(m_1,\pi_1), (m_2,\pi_2)$,  as inputs. If $m_1,m_2$ have a common-prefix with length $\lambda$, and $\pi_1,\pi_2$ are generated from the same certificate, it outputs $1$; otherwise outputs $0$.
      \end{enumerate}


      
  \smallskip
  The first one characterizes a special {\em accountability} requirement in anonymous authentication. It requires that no efficient adversary can authenticate two messages with a common-prefix without being linked, if using the same certificate. More generally, if an attacker corrupts $q$ users, she cannot authenticate $q+1$ messages sharing a common-prefix, without being noticed.  Formally, consider the following cryptographic game between a challenger $\cC$ and an attacker $\cA$:
  \begin{enumerate}
      \item $\cSetup$. The challenger $\cC$ runs the $\cSetup$ algorithm and obtains the master keys.    
      \item $\cCertGen$ queries. The adversary $\cA$ submits $q$ public keys with different identities and obtains $q$ different certificates: $cert_1,\ldots,cert_q$.
      \item $\Auth$. The adversary $\cA$ chooses $q+1$ messages $p||m_1,\ldots,p||m_{q+1}$ sharing a common-prefix $p$ (with $|p|=\lambda$) and authenticates to the challenger $\cC$ by generating the corresponding attestations $\pi_1,\ldots,\pi_{q+1}$.
      \end{enumerate}
Adversary $\cA$ wins if all $q+1$ authentications pass the verification, and no pair of those authentications were linked.
  
      
      \theoremstyle{definition}
      \begin{definition}[Common-prefix-linkability]		For all probabilistic polynomial time algorithm $\huaA$, $\Pr[\huaA $ wins in the above game$]$ is negligible on the security parameter $\lambda$.
      \label{def:linkable} 


      \end{definition}
  

     
     
     Next is the {\em anonymity} guarantee in normal cases. We would like to ensure the anonymity against any party, including the public, the registration authority, and the verifier who can ask for multiple (and potentially correlated) authentication queries. Also, our strong anonymity requires that no one can even link whether the same people is authenticating for different messages, if these messages have different prefixes. The basic requirement for anonymity is that no one can recognize the real identity from the authentication transcript. But our {\em unlinkability} requirement is strictly stronger, as if one can recognize identity, obviously, she can link two authentications by first recovering the actual identities. 
     
     \smallskip
     To capture the unlinkability (among the authentications of different-prefix messages), we can imagine the most  stringent setting, where there are only two honest users in the system,  the adversary still cannot properly link any of them from a sequence of authentications. Formally, consider the following game between the challenger $\cC$ and adversary $\cA$.
      %
      \begin{enumerate}
      \item $\cSetup$.  The adversary $\cA$  generates the master key pair.    
      \item $\cCertGen$. The adversary $\cA$ runs the certificate generation procedure as a registration authority with the challenger. The challenger submits two public keys
      $pk_0,pk_1$ and the adversary generates the corresponding certificates for them $cert_0,cert_1$. $\cA$ can always generate certificates for public keys generated by herself.
      \item $\Auth$-queries. The adversary $\cA$ asks the challenger to serially use $(sk_0,pk_0,cert_0)$ and $(sk_1,pk_1,cert_1)$  to do a sequence of authentications on messages chosen by her. Also, the number $q$ of authentication queries is chosen by $\cA$. The adversary obtains $2q$ message-attestation pairs.
      \item $\Challenge$. The adversary $\cA$ chooses a new message $m^*$ which does not have a common prefix with any of the messages asked in the $\Auth$-queries, and asks the challenger to do one more authentication. $\cC$ picks a random bit $b$ and authenticates on $m^*$ using $sk_b,pk_b,cert_b$. After receiving the attestation $\pi_b$, $\cA$ outputs her guess $b'$.
      \end{enumerate}
      
The adversary wins if $b'=b$.
      
      
      
      \theoremstyle{definition}
      \begin{definition}[Anonymity]
      \label{def:unlinkable} 
      		An authentication scheme is unlinkable, if $\forall$ probabilistic polynomial-time algorithm $\huaA$, $|\Pr[\huaA $ wins in the game$] - \frac{1}{2}|$ is negligible. \footnotemark
      \end{definition}
  
      \footnotetext{We remark that our definition of anonymity is strictly stronger than that definition of the event-oriented linkable group signature \cite{ASY06}, in which the RA can revoke user anonymity under certain conditions.}

      
      
	\smallskip
	\noindent{\bf Construction.} Now we proceed to construct such a primitive. Same as many anonymous authentication constructions, we will also use the zero-knowledge proof technique towards anonymity. In particular, we will leverage zk-SNARK to give an efficient construction. For the above concept of \sameprefix-linkable anonymous authentication, we need to further support the special accountability requirement. The idea is as follows, since the condition that ``breaks'' the linkability is common-prefix, thus the authentication will do a special treatment on the prefix. In particular, the authentication shows a tag committing to the prefix together with the user's secret key, and then presents zero-knowledge poof that such a tag is properly formed, i.e., computed by hashing the prefix and a secret key. To ensure other basic security notions, we will also compute the other tag that commits to the whole message. The user will further prove in zero-knowledge that the secret key corresponds to a certified public key.
	
	\smallskip
	We remark that our main goal is to construct a decentralized crowdsourcing, such a new anonymous authentication primitive could be further studied systematically in future works. Concretely, we present the detailed construction as follows:

      \begin{enumerate}
      \item[-] $\cSetup(\lambda)$. This algorithm establishes the public parameters $PP$ that will be needed for the zk-SNARK system. Also, the algorithm generates a key pair $(msk,mpk)$ which is for a digital signature scheme.\footnote{To be more precise, the public parameter generation could be from another algorithm, for simplicity, we put it here. In the security game for anonymity, the adversary only generates the $msk,mpk$, not the public parameter. }
      \item[-]  $\cCertGen(msk,pk_i)$: This algorithm runs a signing algorithm on $pk_i$,\footnote{Here we  assume there is an external identification procedure to check the actual identity with the public key, and the user key pairs are generated using common algorithms, e.g., for a digital signature, here we ignore the details.} and obtains a signature $\sigma_i$. It outputs $cert_i:=\sigma_i$.
      \item[-] $\Auth(p||m,sk_i,pk_i,cert_i,PP)$: On inputing  a message $p||m$ having a prefix $p$. 
      
      The algorithm first computes two tags (or interchangeably called headers later), $t_1=H(p,sk_i)$ and $t_2=H(p||m,sk_i)$, where $H$ is a secure hash function. 
      Then, let $\vec{w}=(sk_i,pk_i,cert_i)$ represent the private witness, and $\vec{x}=(p||m,mpk)$ be all common knowledge, the algorithm runs zk-SNARK proving algorithm $\cProve(\vec{x},\vec{w},PP)$ for the following language $\huaL_{T}:= \{ t_1,t_2,\vec{x} = (p||m,mpk) \mid \exists \vec{w}=(sk_i,pk_i,cert_i)$ s.t. $\cCertVrfy(cert_i,pk_i,mpk)=1 \wedge pair(pk_i,sk_i)=1\wedge t_1 = H(p,sk_i) \wedge t_2=H(p||m,sk_i)\}$, {where the $\cCertVrfy$ algorithm checks the validity of the certificate using a signature verification, and $pair$ algorithm verifies whether two keys are a consistent public-secret key pair}. This prove algorithm yields a proof $\eta$ for the statement $\vec{x} \in \huaL$ (also for the proof-of-knowledge of $\vec{w}$). 
      
      Finally, the algorithm outputs $\pi:=(t_1,t_2,\eta)$.
      
      \item[-] $\Verify(p||m,\pi,mpk,PP)$: this algorithm runs the verifying algorithm of zk-SNARK $\cVerify$ on $\vec{x},\pi$ and $PP$, and outputs the decision bit $d\in\{0,1\}$.
      \item[-] $\Link(m_1,\pi_1,m_2,\pi_2)$: On inputting two attestations $\pi_1:=(t_1^1,t_2^1,\eta_1)$ and $\pi_2:=(t_1^2,t_2^2,\eta_2)$, the algorithm simply checks $t_1^1\stackrel{?}{=}t_1^2$. If yes, output $1$; otherwise, output $0$. We also use $\Link(\pi_1,\pi_2)$ for short.
      \end{enumerate}
    
    \smallskip
    \noindent{\bf Security analysis (sketch).} Here we briefly sketch the security analysis for the above construction. 
    
    \smallskip
  	Regarding {\em correctness}, it is trivial, because of the completeness of the underlying SNARK.  
	


	\smallskip
	Regarding {\em unforgeability}, we require an uncertified attacker cannot authenticate. The only transcripts can seen by the adversary are headers and the zero-knowledge attestation. Headers include one generated by hashing the concatenation of $p||m,sk$. In order to provide a header, the attacker has to know the corresponding $sk$, as it can be extracted in the random oracle queries. Thus there are only two different ways for the attacker: (i) the attacker generates forges the certificate, which clearly violates the signature security; (ii) the attacker forges the attestation using an invalid certificate, which clearly violates the proof-of-knowledge of the zk-SNARK.
	
	\smallskip
	Regarding the {\em common-prefix-linkability}, it is also fairly straightforward, as the final authentication transcript contains a header  computed by $H(p,sk)$ which is an invariable for a common prefix $p$ using the same secret key $sk$. 

  	\smallskip
  	Regarding the {\em anonymity/unlinkability}, we require that after seeing a bunch of authentication transcripts from one user, the attacker cannot figure out whether a new authentication comes from the same user. This holds even if the attacker can be the registration authority that issues all the certificates. To see this, as the attacker will not be able to figure the value of the $sk$ from all public value, thus the headers/tags can be considered as random values. It follows that $H(p,sk)$ and a random value $r$ cannot be distinguished (similarly for $H(p||m,sk)$). More importantly, due to the zero-knowledge property of zk-SNARK, given $r$, a simulator can simulate a valid proof $\eta^*$ by controlling the common reference string of the zk-SNARK. That said, the public transcript $t_1,t_2,\eta$ can be simulated by $r_1,r_2,\eta^*$ where $r_1,r_2$ are uniform values, and $\eta^*$ is a simulated proof, all of which has nothing to do with the actual witness $sk$. 
  	
  	\smallskip
  	Summarizing the above intuitive analysis, we have the following theorem:

  	
  		
  	\begin{theorem}
  			Conditioned on that the hash function to be modeled as a random oracle and the zk-SNARK is zero-knowledge, the construction of the common-prefix-linkable anonymous authentication satisfies anonymity. Conditioned on the underlying digital signature scheme used is secure, and the zk-SNARK satisfies proof-of-knowledge, our construction of the common-prefix-linkable anonymous authentication will be unforgeable. It is also correct and common-prefix linkable.
  	\end{theorem}




